A Comprehensive Survey of Deep Learning for Time Series Forecasting: Architectural Diversity and Open Challenges

Time series forecasting is a critical task that provides key information for decision-making. After traditional statistical and machine learning approaches, various fundamental deep learning architectures such as MLPs, CNNs, RNNs, and GNNs have been developed. However, the structural limitations caused by the inductive biases of each deep learning architecture constrained their performance. Transformer models, which excel at handling long-term dependencies, have become significant architectural components for time series forecasting. However, recent research has shown that alternatives such as simple linear layers can outperform Transformers. These findings have opened up new possibilities for using diverse architectures, ranging from fundamental deep learning models to emerging architectures and hybrid approaches. In this context, architectural modeling of time series forecasting has now entered a renaissance. This survey not only provides a historical context for time series forecasting but also offers comprehensive and timely analysis of the movement toward architectural diversification. By comparing and re-examining deep learning models, we uncover new perspectives and present recent trends, including hybrid, diffusion, Mamba, and foundation models. By focusing on the inherent characteristics of time series data, we also address open challenges that have gained attention in time series forecasting, such as channel dependency, distribution shift, causality, and feature extraction. These contributions help lower entry barriers for newcomers by providing a systematic understanding of the diverse research areas in time series forecasting (TSF), while offering seasoned researchers broader perspectives and new opportunities through in-depth exploration of TSF challenges. (Shortened due to arXiv's 1,920-character limit. Full version in the paper.)

==> Appendices.tex <==
% An appendix contains supplementary information that is not an essential part of the text itself but which may be helpful in providing a more comprehensive understanding of the research problem or it is information that is too cumbersome to be included in the body of the paper.

% \section{Monash Time Series Forecasting Archive}\label{secA}

% \setcounter{table}{13} % 본문에서 마지막 표 번호로 설정
% \renewcommand{\thetable}{\arabic{table}} % 일반적인 번호 체계를 사용


% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline
% \rowcolor[HTML]{808080} 
% \textbf{Dataset} & \textbf{Domain} & \textbf{No: of Series} & \textbf{Min. Length} & \textbf{Max. Length} & \textbf{Competition} & \textbf{Multivariate} & \textbf{Download} & \textbf{Source} \\ \hline
% M1                     & Multiple  & 1001    & 15   & 150    & Yes  & No  & Yearly, Quarterly, Monthly          & Makridakis et al., 1982          \\ \hline
% M3                     & Multiple  & 3003    & 20   & 144    & Yes  & No  & Yearly, Quarterly, Monthly, Other   & Makridakis and Hibon, 2000       \\ \hline
% M4                     & Multiple  & 100000  & 19   & 9933   & Yes  & No  & Yearly, Quarterly, Monthly, Weekly, Daily, Hourly & Makridakis et al., 2020          \\ \hline
% Tourism                & Tourism   & 1311    & 11   & 333    & Yes  & No  & Yearly, Quarterly, Monthly          & Athanasopoulos et al., 2011      \\ \hline
% CIF 2016               & Banking   & 72      & 34   & 120    & Yes  & No  & Monthly                             & Stepnicka and Burda, 2017        \\ \hline
% London Smart Meters    & Energy    & 5560    & 288  & 39648  & No   & No  & W Missing, W/O Missing              & Jean-Michel, 2019                \\ \hline
% Aus. Electricity Demand& Energy    & 5       & 230736 & 232272 & No   & No  & Half Hourly                         & Curated by us                    \\ \hline
% Wind Farms             & Energy    & 339     & 6345 & 527040 & No   & No  & W Missing, W/O Missing              & Curated by us                    \\ \hline
% Dominick               & Sales     & 115704  & 28   & 393    & No   & No  & Weekly                              & James M. Kilts Center, 2020      \\ \hline
% Bitcoin                & Economic  & 18      & 2659 & 4581   & No   & No  & W Missing, W/O Missing              & Curated by us                    \\ \hline
% Pedestrian Counts      & Transport & 66      & 576  & 96424  & No   & No  & Hourly                              & City of Melbourne, 2020          \\ \hline
% Vehicle Trips          & Transport & 329     & 70   & 243    & No   & No  & W Missing, W/O Missing              & fivethirtyeight, 2015            \\ \hline
% KDD Cup 2018           & Nature    & 270     & 9504 & 10920  & Yes  & No  & W Missing, W/O Missing              & KDD Cup, 2018                    \\ \hline
% Weather                & Nature    & 3010    & 1332 & 65981  & No   & No  & Daily                               & Sparks et al., 2020              \\ \hline
% NN5                    & Banking   & 111     & 791  & 791    & Yes  & Yes & Daily W Missing, Daily W/O Missing, Weekly & Ben Taieb et al., 2012    \\ \hline
% Web Traffic            & Web       & 145063  & 803  & 803    & Yes  & Yes & Daily W Missing, Daily W/O Missing, Weekly & Google, 2017               \\ \hline
% Solar                  & Energy    & 137     & 52560 & 52560  & No   & Yes & 10 Minutes, Weekly                  & Solar, 2020                      \\ \hline
% Electricity            & Energy    & 321     & 26304 & 26304  & No   & Yes & Hourly, Weekly                      & UCI, 2020                        \\ \hline
% Car Parts              & Sales     & 2674    & 51   & 51     & No   & Yes & W Missing, W/O Missing              & Hyndman, 2015                    \\ \hline
% FRED-MD                & Economic  & 107     & 728  & 728    & No   & Yes & Monthly                             & McCracken and Ng, 2016           \\ \hline
% San Francisco Traffic  & Transport & 862     & 17544 & 17544  & No   & Yes & Hourly, Weekly                      & Caltrans, 2020                   \\ \hline
% Rideshare              & Transport & 2304    & 541  & 541    & No   & Yes & W Missing, W/O Missing              & Curated by us                    \\ \hline
% Hospital               & Health    & 767     & 84   & 84     & No   & Yes & Monthly                             & Hyndman, 2015                    \\ \hline
% COVID Deaths           & Nature    & 266     & 212  & 212    & No   & Yes & Daily                               & Johns Hopkins University, 2020   \\ \hline
% Temperature Rain       & Nature    & 32072   & 725  & 725    & No   & Yes & W Missing, W/O Missing              & Curated by us                    \\ \hline
% Sunspot                & Nature    & 1       & 73931 & 73931  & No   & No  & W Missing, W/O Missing              & Sunspot, 2015                    \\ \hline
% Saugeen River Flow     & Nature    & 1       & 23741 & 23741  & No   & No  & Daily                               & McLeod and Gweon, 2013           \\ \hline
% US Births              & Nature    & 1       & 7305 & 7305   & No   & No  & Daily                               & Pruim et al., 2020               \\ \hline
% Solar Power            & Energy    & 1       & 7397222 & 7397222 & No   & No  & 4 Seconds                           & Curated by us                    \\ \hline
% Wind Power             & Energy    & 1       & 7397147 & 7397147 & No   & No  & 4 Seconds                           & Curated by us                    \\ \hline
% \end{tabular}%
% }
% \caption{Summary of Various Datasets in Different Domains}
% \label{tab:dataset_summary}
% \end{table}







\section{Section title of first appendix}\label{secB}

